DiffH2O: Diffusion-Based Synthesis of Hand-Object Interactions from Textual Descriptions

Generating natural hand-object interactions in 3D is challenging as the resulting hand and object motions are expected to be physically plausible and semantically meaningful. Furthermore, generalization to unseen objects is hindered by the limited scale of available hand-object interaction datasets. In this paper, we propose a novel method, dubbed DiffH2O, which can synthesize realistic, one or two-handed object interactions from provided text prompts and geometry of the object. The method introduces three techniques that enable effective learning from limited data. First, we decompose the task into a grasping stage and an text-based manipulation stage and use separate diffusion models for each. In the grasping stage, the model only generates hand motions, whereas in the manipulation phase both hand and object poses are synthesized. Second, we propose a compact representation that tightly couples hand and object poses and helps in generating realistic hand-object interactions. Third, we propose two different guidance schemes to allow more control of the generated motions: grasp guidance and detailed textual guidance. Grasp guidance takes a single target grasping pose and guides the diffusion model to reach this grasp at the end of the grasping stage, which provides control over the grasping pose. Given a grasping motion from this stage, multiple different actions can be prompted in the manipulation phase. For the textual guidance, we contribute comprehensive text descriptions to the GRAB dataset and show that they enable our method to have more fine-grained control over hand-object interactions. Our quantitative and qualitative evaluation demonstrates that the proposed method outperforms baseline methods and leads to natural hand-object motions.

==> sections/FIG/supp_images_p1.tex <==
% \begin{figure*}
% \centering
% \includegraphics[width=1.0\textwidth]{sections/figures/failures_v0.pdf}
% \caption{}
% \label{fig:more_samples}
% \end{figure*}

% \begin{figure*}[t!]
% \centering
% \begin{overpic}
% %, grid, ticks=10
% [width=0.6\textwidth]{sections/figures/qualititative_comparison_v1.pdf}
% \put(0.5,-2.5){\rotatebox{90}{\small{IMoS~\cite{IMoS}}}}
% \put(0.5,32.5){\rotatebox{90}{\small{DiffH$_{2}$O (Ours)}}}
% \put(91, 23.5){{\small{time}}}
% \end{overpic}

% %

% %\caption{\textbf{Qualitative Comparison.} The baseline (bottom row) can exhibit artifacts due to the post-optimized object motions. This often occurs in cases when the object needs to switch hands. Our model (top row) can seamlessly handle hand transitions.}
% \caption{\textbf{Qualitative Comparison.} Post-optimizing object motion as shown in IMoS \cite{IMoS} (bottom row) can exhibit artifacts with fine-grained manipulations, e.g., when an object switches hands.  In contrast, our approach (top row) can seamlessly handle such scenarios. Best seen in the supplemental video.}
% \label{fig:qualitative}
% \end{figure*}



\begin{figure*}[b!]
    \centering

    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/000657_s6_apple_offhand_1.pdf}
        \put(10,90){left hand}
        \put(10, 75){right hand}
        \put(5,5){"The individual hands off the apple."}
        \end{overpic}
        \label{fig:sub1}
    \end{subfigure}
    \hfill % this will insert a non-breakable space between the figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/000018_s1_train_offhand_1.pdf}
         \put(70,30){grasp reference}
         \put(30,10){grasp reference}
        \end{overpic}
        \label{fig:sub2}
    \end{subfigure}
    \hfill % this will insert a non-breakable space between the figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/000190_s1_alarmclock_offhand_1.pdf}
        \put(5,10){"Pick up the alarm clock with the right}
        \put(10,3){hand and pass it to the left hand."}
        \end{overpic}
        \label{fig:sub3}
    \end{subfigure}

    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/000783_s10_pyramidsmall_inspect.pdf}
        \put(0,5){"The person inspects the small pyramid."}
        \end{overpic}
        \caption{Standard Generation}
        \label{fig:sub1}
    \end{subfigure}
    \hfill % this will insert a non-breakable space between the figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/000075_s1_mug_drink_1.pdf}
        \put(70,40){grasp reference}
        \put(55,7){grasp reference}
        \end{overpic}
        \caption{Grasp Guidance}
        \label{fig:sub2}
    \end{subfigure}
    \hfill % this will insert a non-breakable space between the figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/000262_s4_elephant_inspect_1.pdf}
        \put(5,10){"Pick up the elephant with the right}
        \put(5,3){hand and inspect it using both hands."}
        \end{overpic}
        \caption{Comprehensive Texts}
        \label{fig:sub3}
    \end{subfigure}

    \caption{\textbf{Qualitative Examples}. We provide more qualitative examples with a) standard generation without any guidance b) grasp guidance c) our model trained with detailed text descriptions.}
    \label{fig:more_results}
\end{figure*}

% \begin{figure*}[htbp]
% \centering
% \begin{overpic}
% %, grid, ticks=10
% [width=0.9\textwidth]{sections/figures/real_obj_1.pdf}
% \put(32,18){{image-based}}
% \put(32,15){{pose estimator}}
% \put(95.5,19){{{time}}}
% \end{overpic}

% %

% %\caption{\textbf{Qualitative Comparison.} The baseline (bottom row) can exhibit artifacts due to the post-optimized object motions. This often occurs in cases when the object needs to switch hands. Our model (top row) can seamlessly handle hand transitions.}
% \caption{\textbf{Generation from Pose Estimate.} We use an off-the-shelf image based pose estimator to provide a grasp grasp. Our model then generates a variety of different actions that pass through the provided hand pose.}
% \label{fig:ho3d}
% \end{figure*}


\begin{figure*}[htbp]
    \centering

    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/wrong_action_apple_1.pdf}
         \put(10,90){left hand}
         \put(10, 75){right hand}
         \put(10, 5){"Pick up the apple and eat it."}
        \end{overpic}
        \caption{Wrong action}
        \label{fig:fail_sub1}
    \end{subfigure}
    \hfill % this will insert a non-breakable space between the figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/wrong_hand_torus_kf.pdf}
        \put(10,90){left hand}
        \put(50.5,90){grasp reference}
        \put(10, 75){right hand}
        \put(25, 5){"Pass the large torus."}
        \end{overpic}
        \caption{grasp guidance failure}
        \label{fig:fail_sub2}
    \end{subfigure}
    \hfill % this will insert a non-breakable space between the figures
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \begin{overpic}
        [width=\textwidth]{sections/figures/wrong_hand_train_prompt.pdf}
        \put(10,90){left hand}
        \put(10, 75){right hand}
        \put(10, 5){"Pass the train using the left hand."}
        \end{overpic}
        \caption{Handedness failure}
        \label{fig:fail_sub3}
    \end{subfigure}

    \caption{\textbf{Failure Cases}. We present three possible failure cases of our method. a) The generated motion does not match the action described in the input prompt, such as trying to perform a bottle opening motion with an apple. b) During grasp guidance, the reference grasp is largely ignored in the diffusion process, resulting in an interaction that is distinct from the grasp reference. c) Despite training with our curated text annotations, the model sometimes does not pick up on the cue of handedness and may interact with a hand different from the one provided in the text prompt.}
    \label{fig:fail}
\end{figure*}

==> sections/tables/ablation.tex <==
\begin{table}%

\begin{minipage}{\columnwidth}
\begin{center}

\resizebox{1.0\linewidth}{!}{%%
\begin{tabular}{l|ccc|ccc}
   \toprule
    & \multicolumn{3}{c|}{Grasping} & \multicolumn{3}{c}{Articulation} \\
    \midrule
    Models & Suc. G $\uparrow$ & PE $\downarrow$ & AE $\downarrow$ & Suc. A $\uparrow$ & AAE $\downarrow$ & SD $\downarrow$ \\
   \midrule
    w/o curriculum     & \textbf{0.74} & \textbf{0.13} & \textbf{0.65} & 0.36 & 0.77 & 0.02  \\
    w/o cooperation    & 0.21 & 0.32 & 1.43 & 0.48 & 0.65 & 0.02 \\
    w/o art. features  & 0.67 & 0.15 & 0.73 & 0.48 & 0.67 & 0.01 \\
    % No AdaptiveFrame  & - & - & - & 0 & 0 & 0 \\
    \midrule
    Ours             & 0.71 & \textbf{0.13} & 0.69 & \textbf{0.55} & \textbf{0.57} & \textbf{0.01} \\
   \bottomrule
\end{tabular}
}%%

\end{center}

\end{minipage}
\caption{\heading{Ablations} We ablate our curriculum, cooperative training, and the articulation features. All components are important aspects to achieve grasping and articulation with a single policy.}
\label{tab:two}

\end{table}%



==> sections/tables/supp_tab_action_correctness_per_obj.tex <==


\begin{table*}[]
  \centering
    \resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}l|ll|ll|c|cccccccccc@{}}
\toprule
 & \multicolumn{2}{c|}{Split} & \multicolumn{2}{c|}{Textual input form} & \begin{tabular}[c]{@{}c@{}}Action\\ correctness\end{tabular} & \multicolumn{8}{c}{Action correctness over object classes} \\ \midrule
\multicolumn{1}{l|}{Method} & \multicolumn{1}{c}{Train split} & \multicolumn{1}{c|}{Test split} & \multicolumn{1}{c}{Train input} & \multicolumn{1}{c|}{Test input} & Overall & apple & mug & train & \begin{tabular}[c]{@{}c@{}}alarm\\ clock\end{tabular} & elephant & \begin{tabular}[c]{@{}c@{}}medium\\ cylinder\end{tabular} & \begin{tabular}[c]{@{}c@{}}small\\ pyramid\end{tabular} & \begin{tabular}[c]{@{}c@{}}large\\ torus\end{tabular} \\ \midrule
IMOS* & subject & object & simple & simple & 90.3 & 90.9 & 89.5 & 77.8 & \textbf{100} & 80.0 & \textbf{100} & 83.3 & \textbf{100} \\
Ours & subject & object & simple & simple & \textbf{99.5} & \textbf{100} & \textbf{97.4} & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{100} \\
\midrule
Ours & object & object & \multicolumn{1}{c}{simple} & \multicolumn{1}{c}{simple} & 89.7 & 81.8 & 92.1 & 50.0 & 100 & 100 & 100 & 100 & 100 \\
\midrule
Ours & object & object & \multicolumn{1}{c}{simple} & comprehensive & 54.8 & 40.9 & 55.3 & 16.7 & 52.6 & 80.0 & 75 & 50.0 & 68.8 \\ 
Ours & object & object & comprehensive & comprehensive & 93.5 & 95.5 & 94.7 & 77.8 & 100 & 95.0 & 93.6 & 100 & 93.6 \\
\bottomrule
\end{tabular}
  }
 
\caption{\textbf{Details of the Text Evaluation.} Comparison of our method against IMoS and our model's variants that use different forms of textual input. We generate synthetic hand-object  pose sequences from each model based on textual prompts in two forms: a simple ("verb" + "object") and our detailed, proposed GRAB dataset annotations ("comprehensive"). We verify whether the generated sequences feature the correct action. We test all methods on our newly created unseen object split, which excludes 7 object classes for testing.} 
  \label{tab:action_correctness_per_obj}
\end{table*}

==> sections/tables/train_test_splits.tex <==
\begin{table}
\centering
\begin{center}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l|cccc}
   \toprule
        & Subject  & Object  & Semantic  & Num \\
     Method      & Split  & Split  & Based & Unseen Obj  \\
    \midrule
    GRAB    & \redcross    & \greencheck                 & \redcross & 6    \\
    % \rowcolor{Gray}
    IMoS  & \greencheck   & \redcross                 & \redcross & - \\
    \textbf{\methodname\ (Ours)} &  \redcross & \greencheck         & \greencheck & 8  \\
   \bottomrule
\end{tabular}
}
\end{center}
\caption{\heading{Comparison between ours and existing methods} Ours generates two-hand manipulations using physics simulation, requires only static hand pose references (few shot), and accommodates both rigid and articulated objects with a unified policy.}
\label{tab:related_work}
\end{table}

